Efficient Gradient-Based Inference through Transformations between Bayes Nets and Neural Nets

Hierarchical Bayesian networks and neural networks with stochastic hidden units are commonly perceived as two separate types of models. We show that either of these types of models can often be transformed into an instance of the other, by switching between centered and differentiable non-centered parameterizations of the latent variables. The choice of parameterization greatly influences the efficiency of gradient-based posterior inference; we show that they are often complementary to eachother, we clarify when each parameterization is preferred and show how inference can be made robust. In the non-centered form, a simple Monte Carlo estimator of the marginal likelihood can be used for learning the parameters. Theoretical results are supported by experiments.

==> 2014-01_icml14_af copy/commands.tex <==
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsfonts}
%\usepackage{mathtools}

% Draw Bayes nets
% From: https://github.com/jluttine/tikz-bayesnet
\usepackage{tikz}
\usetikzlibrary{bayesnet}

\newcommand{\bb}[1]{\mathbf{#1}}
\newcommand{\bx}{\bb{x}}
\newcommand{\bxi}{\bx^{(i)}}
\newcommand{\bt}{\bb{t}}
\newcommand{\bT}{\boldsymbol{\theta}}
\newcommand{\by}{\bb{y}}
\newcommand{\bv}{\bb{v}}
\newcommand{\bw}{\bb{w}}
\newcommand{\bd}{\bb{d}}
\newcommand{\br}{\bb{r}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\bz}{\bb{z}}
\newcommand{\bpa}{\bb{pa}}
\newcommand{\btpa}{\widetilde{\bb{pa}}}
\newcommand{\bch}{\bb{ch}}
\newcommand{\bL}{\bb{L}}
\newcommand{\bO}{\bb{O}}
\newcommand{\pT}{p_{\bT}}
\newcommand{\bsigma}{\bb{\sigma}}

\newcommand{\ep}{\epsilon}

%\newcommand{\tz}{\widetilde{z}}
%\newcommand{\tZ}{\widetilde{Z}}
%\newcommand{\tf}{\widetilde{f}}
%\newcommand{\btZ}{\widetilde{\bb{Z}}}
%\newcommand{\btz}{\widetilde{\bz}}
%\newcommand{\tPa}{\widetilde{Pa}}
%\newcommand{\btPa}{\widetilde{\bb{Pa}}}

\newcommand{\Exp}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Ed}{\mathbb{E}_\bd}
\newcommand{\eqnr}{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\Lxz}{L^{(\bx,\bz)}}
\newcommand{\Lxe}{L^{(\bx,\beps)}}
\newcommand{\Lzj}{L^{(z_j)}}
\newcommand{\Lz}{L^{(z)}}
\newcommand{\Lnz}{L^{(\setminus z)}}
\newcommand{\Lcz}{L^{(z\rightarrow)}}
\newcommand{\Hnz}{H^{(\setminus z)}}
\newcommand{\Hcz}{H^{(z\rightarrow)}}

\newcommand{\Lej}{L^{(e_j)}}
\newcommand{\LpajOrig}{L_{orig}^{(\bch(z_j)|z_j)}}
\newcommand{\LpajAux}{L_{aux}^{(\bx|z_j)}}

\DeclareMathOperator*{\argmax}{argmax}

% First and second partial derivatives
\newcommand{\fpd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\spd}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}


% Create 'example' environment
\theoremstyle{definition}
\newtheorem{exmp}{Example}[section]



==> 2014-01_icml14_af copy/shared/commands.tex <==
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

% Bold shortcuts
\newcommand{\bb}[1]{\mathbf{#1}}
% - lowercase
\newcommand{\bbb}{\bb{b}}
\newcommand{\bx}{\bb{x}}
\newcommand{\bxi}{\bx^{(i)}}
\newcommand{\bxl}{\bx^{(l)}}
\newcommand{\bt}{\bb{t}}
\newcommand{\by}{\bb{y}}
\newcommand{\bv}{\bb{v}}
\newcommand{\bw}{\bb{w}}
\newcommand{\bc}{\bb{c}}
\newcommand{\bd}{\bb{d}}
\newcommand{\bg}{\bb{g}}
\newcommand{\bh}{\bb{h}}
\newcommand{\br}{\bb{r}}
\newcommand{\bu}{\bb{u}}
\newcommand{\byl}{\by^{(l)}}
\newcommand{\bz}{\bb{z}}
\newcommand{\bzi}{\bz^{(i)}}
\newcommand{\bzl}{\bz^{(l)}}
\newcommand{\bzil}{\bz^{(i,l)}}
\newcommand{\bpa}{\bb{pa}}

\newcommand{\bT}{\boldsymbol{\theta}}
\newcommand{\bTl}{\boldsymbol{\theta}^{(l)}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\bepsl}{\beps^{(l)}}
\newcommand{\bepsil}{\beps^{(i,l)}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bzetal}{\zeta^{(l)}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bzero}{\bb{0}}

% - uppercase
\newcommand{\bL}{\bb{L}}
\newcommand{\bV}{\bb{V}}
\newcommand{\bW}{\bb{W}}
\newcommand{\bI}{\bb{I}}
\newcommand{\bR}{\bb{R}}
\newcommand{\bX}{\bb{X}}
\newcommand{\bO}{\bb{O}}

\newcommand{\btPa}{\widetilde{\bb{Pa}}}
\newcommand{\btpa}{\widetilde{\bb{pa}}}

% Tilde
\newcommand{\tz}{\widetilde{z}}
\newcommand{\tZ}{\widetilde{Z}}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\btZ}{\widetilde{\bb{Z}}}
\newcommand{\btz}{\widetilde{\bz}}
\newcommand{\btT}{\widetilde{\bT}}
\newcommand{\tPa}{\widetilde{Pa}}

\newcommand{\pT}{p_{\bT}}
\newcommand{\pTl}{p_{\bT^{(l)}}}
\newcommand{\pA}{p_{\balpha}}
\newcommand{\qT}{q_{\bT}}
\newcommand{\qPhi}{q_{\bphi}}
\newcommand{\fT}{f_{\bT}}
\newcommand{\fPhi}{f_{\bphi}}
\newcommand{\fTPhi}{f_{\bT,\bphi}}
\newcommand{\gT}{g_{\bT}}
\newcommand{\gPhi}{g_{\bphi}}
\newcommand{\hPhi}{h_{\bphi}}

\newcommand{\Exp}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Ed}{\mathbb{E}_\bd}
\newcommand{\eqnr}{\addtocounter{equation}{1}\tag{\theequation}}

\DeclareMathOperator*{\argmax}{argmax}

% Create 'example' environment
\theoremstyle{definition}
\newtheorem{exmp}{Example}[section]

% Variational bound
\newcommand{\LB}[2]{\mathcal{L}^{#1}(\bT,\bphi; #2)}
\newcommand{\LBT}[2]{\widetilde{\mathcal{L}}^{#1}(\bT,\bphi; #2)}


==> 2014-01_icml14_af copy/tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}



==> shared/commands.tex <==
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

% Bold shortcuts
\newcommand{\bb}[1]{\mathbf{#1}}
% - lowercase
\newcommand{\bbb}{\bb{b}}
\newcommand{\bx}{\bb{x}}
\newcommand{\bxi}{\bx^{(i)}}
\newcommand{\bxl}{\bx^{(l)}}
\newcommand{\bt}{\bb{t}}
\newcommand{\by}{\bb{y}}
\newcommand{\bv}{\bb{v}}
\newcommand{\bw}{\bb{w}}
\newcommand{\bc}{\bb{c}}
\newcommand{\bd}{\bb{d}}
\newcommand{\bg}{\bb{g}}
\newcommand{\bh}{\bb{h}}
\newcommand{\br}{\bb{r}}
\newcommand{\bu}{\bb{u}}
\newcommand{\byl}{\by^{(l)}}
\newcommand{\bz}{\bb{z}}
\newcommand{\bzi}{\bz^{(i)}}
\newcommand{\bzl}{\bz^{(l)}}
\newcommand{\bzil}{\bz^{(i,l)}}
\newcommand{\bpa}{\bb{pa}}

\newcommand{\bT}{\boldsymbol{\theta}}
\newcommand{\bTl}{\boldsymbol{\theta}^{(l)}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\bepsl}{\beps^{(l)}}
\newcommand{\bepsil}{\beps^{(i,l)}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bzetal}{\zeta^{(l)}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bzero}{\bb{0}}

% - uppercase
\newcommand{\bL}{\bb{L}}
\newcommand{\bV}{\bb{V}}
\newcommand{\bW}{\bb{W}}
\newcommand{\bI}{\bb{I}}
\newcommand{\bR}{\bb{R}}
\newcommand{\bX}{\bb{X}}
\newcommand{\bO}{\bb{O}}

\newcommand{\btPa}{\widetilde{\bb{Pa}}}
\newcommand{\btpa}{\widetilde{\bb{pa}}}

% Tilde
\newcommand{\tz}{\widetilde{z}}
\newcommand{\tZ}{\widetilde{Z}}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\btZ}{\widetilde{\bb{Z}}}
\newcommand{\btz}{\widetilde{\bz}}
\newcommand{\btT}{\widetilde{\bT}}
\newcommand{\tPa}{\widetilde{Pa}}

\newcommand{\pT}{p_{\bT}}
\newcommand{\pTl}{p_{\bT^{(l)}}}
\newcommand{\pA}{p_{\balpha}}
\newcommand{\qT}{q_{\bT}}
\newcommand{\qPhi}{q_{\bphi}}
\newcommand{\fT}{f_{\bT}}
\newcommand{\fPhi}{f_{\bphi}}
\newcommand{\fTPhi}{f_{\bT,\bphi}}
\newcommand{\gT}{g_{\bT}}
\newcommand{\gPhi}{g_{\bphi}}
\newcommand{\hPhi}{h_{\bphi}}

\newcommand{\Exp}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Ed}{\mathbb{E}_\bd}
\newcommand{\eqnr}{\addtocounter{equation}{1}\tag{\theequation}}

\DeclareMathOperator*{\argmax}{argmax}

% Create 'example' environment
\theoremstyle{definition}
\newtheorem{exmp}{Example}[section]

% Variational bound
\newcommand{\LB}[2]{\mathcal{L}^{#1}(\bT,\bphi; #2)}
\newcommand{\LBT}[2]{\widetilde{\mathcal{L}}^{#1}(\bT,\bphi; #2)}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


